A Security and Usability Analysis of Local Attacks Against FIDO2

The FIDO2 protocol aims to strengthen or replace password authentication using public-key cryptography. FIDO2 has primarily focused on defending against attacks from afar by remote attackers that compromise a password or attempt to phish the user. In this paper, we explore threats from local attacks on FIDO2 that have received less attention -- a browser extension compromise and attackers gaining physical access to an HSK. Our systematic analysis of current implementations of FIDO2 reveals four underlying flaws, and we demonstrate the feasibility of seven attacks that exploit those flaws. The flaws include (1) Lack of confidentiality/integrity of FIDO2 messages accessible to browser extensions, (2) Broken clone detection algorithm, (3) Potential for user misunderstanding from social engineering and notification/error messages, and (4) Cookie life cycle. We build malicious browser extensions and demonstrate the attacks on ten popular web servers that use FIDO2. We also show that many browser extensions have sufficient permissions to conduct the attacks if they were compromised. A static and dynamic analysis of current browser extensions finds no evidence of the attacks in the wild. We conducted two user studies confirming that participants do not detect the attacks with current error messages, email notifications, and UX responses to the attacks. We provide an improved clone detection algorithm and recommendations for relying part

==> Implementation.tex <==
\section{Implementation}

We implemented a prototype to demonstrate the feasibility of system and performed performance analysis. In our prototype we worked on three entities:


\begin{figure*}[ht]
\centerline{\includegraphics[width=0.98\textwidth]{images/SGX_FIDO2_implementation.png}}
\caption{Implementation design}
\label{system_overview}
\end{figure*}

\subsection{Secure WebAuthn client}
  We implemented our webAuthn client as a native C application using Yubico's libfido2 library. We implemented the module called Verifier within the native application. The Verifier uses v2.7 of Intel's SGX driver, SDK, and Platform Software(PSW). This native application launches Verifier's secure enclave, which communicates with RP and the authenticator to create a secure channel. This native application directly communicates to the authenticator using the CTAP protocol implemented in the libfido2 library. To allow the app's communication to an RP through a web browser, we implemented a chrome extension. The chrome extension overrides the inbuilt $navigator.credentials.create()$ and $navigator.credentials.get()$ functions, and calls the native app implementation. 
    
    Native app's APIs that are available to the chrome extension/RP are:
    \begin{itemize}
        \item remote attestation of the Verifier secure enclave: The remote attestation process provides the Verifier and the Relying Party with the shared secret key (Sk).
        \item registers an authenticator: If the remote attestation is successful, the input to this API is encrypted by Sk. The Verifier secure enclave decrypts the request and re-encrypts it with the secret key shared with the authenticator.
        \item authentication: same process as registration API.
    \end{itemize}
    
    There is only one native app's API available to the authenticator. The app allows the authenticator to attest to the Verifier's secure enclave. The app also sends the IAS report to the authenticator that helps the authenticator complete the attestation process. The Verifier communicates with the authenticator over an encrypted channel by using the secret key they shared during attestation.  
    
   
\subsection{Relying party}
  In our prototype, we use Yubico's java-webauthn-server to implement an RP. On the server-side, we implemented a separate module $RP checker$. Its primary job is to verify the Verifier's secure enclave through remote attestation and share a secret key $Sk$. It also communicates with IAS to retrieve attestation reports. After succesful attestation, $RP checker$ shares the key $Sk$ with the $RP$. The $RP$ communicates to the webAuthn client over a secure channel encrypted by $Sk$.
  
  \tarun{The authenticator can use the same IAS report that RP uses for itself. Verify it through implementation, if works change the implementation diagram}



\subsection{Authenticator}
TODO

==> System_design.tex <==
\section{v-FIDO2 System Design}

Our goal is to strengthen the security of FIDO2 \hsk{s} against MITM attacks, phishing attacks, and device cloning attacks without sacrificing usability.
We propose Verified FIDO2 (v-FIDO2), a system designed to detect or prevent the attacks described in our threat model. 

More specifically, v-FIDO2 will:
\begin{itemize}
\item Prevent the registration of a malicious \hsk on a FIDO2 security-token-enabled account.
\item Allow the client to use a FIDO2 \hsk only for web services where the owner of the \hsk initiates a login.
\item Support ``remember this device" convenience without the risk of a passive attacker intercepting data (e.g., a cookie) that enables them to impersonate the victim.
\item Detect stealthy device cloning attacks.
\end{itemize}

\subsection{v-FIDO2 Security Model}

The v-FIDO2 design introduces a new security model for the use of FIDO2 \hsk{s} (see Figure~\ref{system_overview}).

The current security model for {\hsk}s assumes a trusted client that communicates with the \rp over TLS and communicates with the \hsk in plaintext.

\begin{figure}[htbp]
\centerline{\includegraphics[width=0.5\textwidth]{images/FIDO2_high_level_design_changes.png}}
\caption{v-FIDO2 Security Model}
\label{system_overview}
\end{figure}

The v-FIDO2 security model introduces a new component, known as the {\em Verifier} (\ver), that runs in a Trusted Execution Environment (TEE) on the same host as the client. The client is assumed to be untrusted. The \rp and the \hsk send only authenticated messages to \ver, which the untrusted client cannot modify without detection. The client and \ver communicate with each other via plaintext messages.

\ver is responsible for (1) maintaining the integrity of the communication between the \rp and the \hsk, (2) executing critical functions securely, such as origin checking, and (3) providing "remember this device" functionality. 
The client's primary responsibility is to set up the verifier's TEE and relay authenticated messages to and from the verifier.  

\subsection{Adding a Security Key Display}

We propose a display screen on the \hsk to help prevent some critical attacks (see Threat Analysis in Section~\ref{analysis}) by involving the user. 
During registration, the \hsk displays information and asks the user to confirm the registration process.

On receiving a registration request, the \hsk displays four items.
\begin{itemize}
    \item \rp name: To confirm that the \hsk is connected to the same RP that the user wants to register with.
    \item Username: To confirm that the \hsk is bound to the intended account at the \rp.
    \item First authenticator/Non-first authenticator: An indicator for whether an \hsk is already bound to this account or not.
    \item Secure enclave/No secure enclave: An indicator for whether the connection involves a secure enclave or not.
\end{itemize}
        
The user taps the \hsk to confirm the details. On confirmation, the \hsk generates the response and sends it to the \rp. 

% \ks{This seems outdated since we replace the counter. Should this be deleted?} If the secure enclave is used, according to our design, the \hsk waits for the acknowledgment from \rp and then increments the clone detection counter and displays confirmation on display. Otherwise, it follows the existing protocol.

\subsection{Virtual Hardware Authenticator}

The verifier (\ver) also provides a ``Remember this device" feature that is resistant to a MITM attack. Once a user authenticates using an \hsk on a device, the user can enable a software \hsk that operates from within \ver and serves as a virtual \hsk. The user can skip hardware authentication for future logins from this device based on the remember me period, avoiding having to insert an \hsk for each authentication. 

\ver creates a private-public key pair used for signing the challenges received from the \rp for authentication. \ver seals the private key, and only \ver can unseal that private key and authenticate. At the time of authentication, \ver first checks whether it has a sealed registered key before prompting the user to authenticate using their \hsk. If the remember me feature has been enabled, \ver uses the sealed key to automatically authenticate in the background.

The use of a virtual \hsk from secure hardware is more secure than passwords, cookies, or shared keys because it preserves the strengths of the authenticator approach (phishing attack resistance, MITM attack prevention, etc.). Unlike cookies, there is no data for an eavesdropper to steal and replay to impersonate the user. Also, the TEE prevents malware from accessing the private key.

\subsection{Registration Acknowledgement}

Currently, the \hsk assumes a complete registration as soon as it sends the response to the client. We propose that the \rp sends an acknowledgment of successful registration back to the \hsk after receiving a valid registration response. The acknowledgement contains the hash of the response from the \hsk. The acknowledgment allows the \hsk to have an accurate status of the registration process. 

\subsection{Hashed Challenge Set}

We propose to replace the current counters stored at the \rp and \hsk with a new mechanism that provides improved detection of cloning attacks.

The \hsk (see Algorithm 1) saves a hash of the challenge it receives during registration as $hashC$.
Upon receipt of an authentication request, the \hsk includes $hashC$ in the response, and updates the hash using the challenge in the authentication request ($hashC = hash(request.Challenge)$).

\begin{algorithm}

\begin{pseudo}
onReceivingRegistrationRequest(request) \\+
    $hashC = hash(request.Challenge)$ \\-
    \\
    
onReceivingAuthenticationRequest(request, hashC) \\+
    $response = generateAuthenticationResponse(hashC)$ \\
    $hashC = hash(request.Challenge)$
    
\end{pseudo}
  \caption{The Hardware Security Key}
\end{algorithm}



The \rp  (see Algorithm 2) maintains a set of the hashed challenges that it sends to the \hsk. 
The \rp initially inserts $hash(request.Challenge)$ in the set when registration completes.
The \rp inserts a hash of the challenge sent in each authentication request. 
Upon receipt of an authentication response, 
the \rp first verifies that the hashed challenge in the response is a member of the set. 
If so, the \rp then clears the set and inserts a hash of the request challenge corresponding to the response that was just received.
If not, then a cloning attack is detected.

\begin{algorithm}
\begin{pseudo}
onReceivingRegistrationResponse(request, response) \\+
    $bufferSet = set()$ \\
    $bufferSet.insert(hash(request.Challenge))$ \\-
    \\


onSendingAuthenticationRequest(request) \\+
    $bufferSet.insert(hash(request.challenge))$ \\-
    \\

onReceivingAuthenticationResponse(request, response) \\+
    $hashC = response.hashC$ \\
    if $hashC$ in $bufferSet$ \\+
        $bufferSet.clear()$ \\
        $bufferSet.insert(hash(request.Challenge))$ \\
        continue $authentication$ \\-
    else \\+
        $cloning$ $detected$ \\-
\end{pseudo}
\caption{The Relying Party}
\end{algorithm}


Since each hashed challenge can only be used once to authenticate, a existence of a cloned \hsk is detected when either device supplies the cloned hash value the second time to the \rp. 

The cloned device has a $1/n$ ($n$ equals the number of bits in the hash) probability of guessing a valid hash in order to authenticate if the original \hsk authenticates first. Even if a guess succeeds, the attack will be detected the next time the valid \hsk authenticates.

The v-FIDO2 design is effective in detecting cloning attacks, and avoids false positives and false negatives in the case that requests or responses are lost during transit.

\begin{itemize}
\item Suppose an authentication request (\rp->\hsk) is lost. Assume that \rp and \hsk each store hashes of $challenge_{i-1}$. When the \rp sends $challenge_i$, it stores a hash of that challenge in the buffer. If that challenge never arrives at the \hsk, the next request will contain $challenge_{i+1}$. The \hsk will return a hash of $challenge_{i-1}$ in the response and store a hash of $challenge_{i+1}$. The \rp will match $challenge_{i-1}$ in the buffer, clear the buffer, and save a hash of $challenge_{i+1}$ in the buffer. 

\item Suppose an authentication response (\hsk->\rp) is lost.
Assume that \rp and \hsk each store hashes of $challenge_{i-1}$. When the \rp sends $challenge_i$, it stores a hash of that challenge in the buffer. The \hsk will return a hash of $challenge_{i-1}$ in the response and store a hash of $challenge_i$. I the response never arrives, the \rp will send $challenge_{i+1}$ in the next request and store a hash of the challenge in the buffer. The \hsk will respond with $challenge_i$ in the response, and store a hash of $challenge_{i+1}$. Upon receipt of a hash of $challenge_i$ in the response, the \rp will clear the buffer, and save a hash of $challenge_{i+1}$ in the buffer. 

\end{itemize}

\subsection{Additional Authenticator Registration}

We propose that an \rp require the user to first authenticate using an existing \hsk when adding an additional \hsk to an account, 
The extra authentication layer prevents an attacker from registering a fake \hsk in the background without the user's knowledge.    

\subsection{Error Messages}

Currently, the \rp assumes responsibility for displaying messages when errors occur during the registration or authentication process.  A malicious phishing website can abuse this privilege and display misleading errors to a user even when the user possesses a valid \hsk.

From our analysis, \rp error messages can be difficult for users to understand.
We propose that the client be responsible for displaying FIDO2 error messages based on standardized error codes and error messages that the \rp returns to the client when an error occurs. 
This approach may be more usable by providing consistent error messages across all relying parties.

For example, when a cloning attack is detected, a standard \emph{Device cloning detected} error code can be returned to the client that results in a standard error messages such as "Your security key may have been cloned. An attacker may have accessed your account. Remove the security from this account and re-register it in order to lock the attacker out."

\section{Prototype Implementation}

We created a prototype implementation of v-FIDO2 using an Intel SGX Enclave module. When a user initiates a registration request, the client initializes the enclave and launches the verifier (\ver).
The \rp and \hsk both attest to {\ver}'s validity using the remote attestation feature of Intel SGX. 
The result of attestation is that \ver shares a secret key with \rp and \hsk respectively. The keys are used to authenticate messages sent between them.

%\subsubsection{Background: Intel SGX}
Intel SGX is a set of CPU instructions that can be used by applications to create an isolated region of memory called an enclave. The enclave is inaccessible to everyone outside the enclave, including processes with admin privileges and the operating system. 
The application that creates an enclave is divided into a trusted and untrusted section. The untrusted section is responsible for creating an enclave and communicating with the rest of the system. 
%The untrusted section uses ECALLs to invoke a pre-defined function, passing input parameters and pointers to shared memory in the enclave. The enclave uses OCALLs to invoke functions outside the enclave by copying input parameters outside the enclave.
    
\paragraph{Remote attestation}
Remote attestation is used to guarantee the integrity of the trusted code in the enclave. When an ISV (Independent Software Vendor) develops the application, they generate a cryptographic hash (known as MRENCLAVE) of the running enclave, including both the code and data of the trusted section. 
The hash is shared with the service providers that need to attest to the enclave of that application. A service provider challenges an enclave to generate a MRENCLAVE and compares it with the MRENCLAVE provided by the ISV.

To verify that the MRENCLAVE is created by a legitimate enclave instance, it must be signed with the Enclave's private key. Relying parties send the signature to the IAS (Intel Attestation Service) for verification.

\subsection{Client and Verifier (\ver)}

We implementeded \ver as an Intel SGX module based on code provided at https://github.com/intel/sgx-ra-sample. 
The client acts as a relay for \hsk-to-\ver and \ver-to-\rp communications. 
We implemented the client in two modules: (1) \textit{browser extension}, responsible for overriding the current FIDO2 browser client and acting as a relay between \rp and the client's native C++ app, and (2) native C++ app that initializes \ver and acts as a relay for client's browser extension-to-\ver and \ver-to-\hsk communication.


 We implemented webAuthn client as a native C/C++ application using Yubico's libfido2 library. We implemented the Intel SGX module ~\ver within the native application based on code provided at https://github.com/intel/sgx-ra-sample. The ~\ver uses v2.7 of Intel's SGX driver, SDK, and Platform Software(PSW). This native application initializes \ver and acts as a relay for \rp-to-\ver and \ver-to-\hsk communication. . It communicates to the ~\hsk using the CTAP protocol implemented in the libfido2 library. To allow the app's communication to an RP through a web browser, we implemented a chrome extension. The chrome extension overrides the inbuilt $navigator.credentials.create()$ and $navigator.credentials.get()$ functions, and calls the native app implementation. 
 
    Native app's APIs that are available to the chrome extension/RP are:
    \begin{itemize}
        \item remote attestation of the ~\ver: The remote attestation process provides the ~\ver and the Relying Party with the shared secret key (Sk).
        \item registers an ~\hsk: If the remote attestation is successful, the input to this API is encrypted by Sk. The ~\ver decrypts the request and re-encrypts it with the secret key shared with the ~\hsk.
        \item authentication: same process as registration API.
    \end{itemize}
    
    There is only one native app's API available to the authenticator. The app allows the authenticator to attest to the Verifier's secure enclave. The app also sends the IAS report to the authenticator that helps the authenticator complete the attestation process. The Verifier communicates with the authenticator over an encrypted channel by using the secret key they shared during attestation.  



\subsection{Hardware Securrity Key (\hsk)}

In our design, the \hsk uses a modified version of the Intel SGX remote attestation process to verify that it is communicating to a valid enclave. Typically a portion of this process requires the service provider, the system requesting proof of an enclave, to connect to the IAS and receive an attestation report. Since the \hsk cannot connect directly to the IAS, the enclave itself retrieves the attestation report and forwards it to the \hsk. The \hsk then verifies the report using the IAS public key that is hard-coded on the device. This process provides evidence to the \hsk that it is authenticated to a genuine SGX enclave and that the enclave is running a valid copy of \ver. After the remote attestation process is completed, each message that is sent between the \hsk and \ver running on the SGX is authenticated using a shared key that is generated during the remote attestation process.


\subsection{Relying Party (\rp)}

The \rp also uses remote attestation to verify it is talking to a valid SGX that is running a valid copy of \ver, resulting in a shared key between \rp and \ver. 
\rp authenticates all messages sent from \ver using that shared key. \rp also sends an acknowledgement after registration or authentication completes successfully.
In our prototype, we build upon Yubico's java-webauthn-server to implement our server. On the server, we implemented a separate module $RP checker$. Its primary job is to verify the \ver secure enclave through remote attestation and share a secret key $Sk$. It also communicates with the \textit{IAS} to retrieve the attestation report. After successful attestation, $RP checker$ shares the key $Sk$ with the $RP$. The webauthn server uses $Sk$ to generate an HMAC of the request and include it in the registration or authentication request.





==> System_design2.tex <==
% \subsubsection{v-FIDO2 System Design}
% We propose Verified FIDO2 (v-FIDO2), a system to strengthen the security of FIDO2 \hsk{s} against MITM attacks, phishing attacks, and device cloning attacks. The goals of the system are:

% \begin{itemize}[topsep=1pt,noitemsep,leftmargin=1.5em]
% \item Prevent the registration of a malicious \hsk on a FIDO2 security-token-enabled account.
% \item Allow the webAuthn client to authenticate using an \hsk only for web services where the owner initiated a login.
% \item Support \textit{remember this device} convenience without running the risk of a passive attacker intercepting data (e.g., a cookie)  and impersonating the victim.
% \item Detect stealthy device cloning attacks.
% \end{itemize}

       
\subsection{WebAuthn API Architecture Improvements Leveraging TEE}
In this defense, we move the webAuthn client to a TEE. Leveraging TEE provides integrity for communications between the \hsk and the webserver. 
% \st{Thus, it also defends against other stronger adversaries like OS and TLS proxies. We first define the stronger adversary model and then present the defense.} 
The following paragraphs explain v-FIDO2's security model, the clone detection algorithm, and the v-FIDO2 protocol entities: \rp, webAuthn client, and \hsk.

\paragraph{v-FIDO2 security model}
The v-FIDO2 design introduces a new security model for FIDO2 \hsk{s} (see Figure~\ref{system_overview}).
The current security model assumes a trusted webAuthn client that communicates with the \rp over TLS and the \hsk in plaintext. The v-FIDO2 security model introduces a new component, the {\em Verifier} (\ver), that runs in a Trusted Execution Environment (TEE) on the same host as the client. The client is assumed to be untrusted. The \rp and the \hsk send only authenticated messages to \ver, which the untrusted client cannot modify without detection.

\begin{figure}[htbp]\centerline{\includegraphics[width=0.5\textwidth]{images/FIDO2_high_level_design_changes.png}}
\caption{v-FIDO2 Security Model}
\label{system_overview}
\end{figure}

\ver is responsible for (1) maintaining communication integrity between the \rp and the \hsk, (2) executing critical functions securely (e.g., origin checking), and (3) providing \textit{remember this device} functionality. The webAuthn client's primary responsibility is to set up \ver's TEE and relay authenticated messages to and from \ver.  

\textit{Adversary model for v-FIDO2}: The adversary controls the victim's webAuthn client, the browser, and the operating system and can execute a MiTM attack on a TLS connection between the victim's client and the server.

\textit{Why consider stronger threat model for v-FIDO2}: 
We design and evaluate v-FIDO2 under a much stronger threat model than what we used to demonstrate attacks in Section ~\ref{sec:attacks}. Section ~\ref{sec:adversary_model} considered only browser extensions in the threat model, which is more realistic to demonstrate the attacks.
However, we believe the defense should be designed under a rigorous threat model. The following example supports our claim of requiring a more robust threat model for v-FIDO2.
Assume a user authenticates to ${\rp}_1$ through \hsk on {\A}'s machine and there is a malware in the OS or the browser. \A could authenticate as victim to ${\rp}_2$, where ${\rp}_2$ is a website that victim is registered with using \hsk (as described in \ref{para:sync_login}).


% v-FIDO2 assumes a stronger threat model than described in Section ~\ref{sec:adversary_model}. 

% We design and evaluate v-FIDO2 under a much stronger threat model than what we used to demonstrate attacks in Section ~\ref{sec:attacks}. Section ~\ref{sec:adversary_model} considered only browser extensions in the threat model, which is more realistic to demonstrate the attacks. However, we believe the defense should be designed under a rigorous threat model.  



\paragraph{Challenges:}
Below are some challenges that we faced while designing a defense using TEE:
\begin{itemize}
    \item How to prove to the user that they are dealing with a trusted application when trusted and untrusted applications share the same display? In our design, we address it by moving the display to the authenticator device.
    \item Cuckoo attack: Preventing MITM by webAuthn client during registration: Remote attestation verifies a valid secure enclave. However, it could be running on any machine. The webAuthn client can redirect the request to the attacker's machine secure enclave. We use registration acknowledgment and display that information to the user to get confirmation.
    \item The attesting party needs to connect to Intel Attestation Service (IAS) through the Internet for the remote attestation process. However, in our case, the \hsk cannot connect to the Internet. In our design, the webserver retrieves the verification report from IAS on behalf of \hsk. The \hsk verifies the report's integrity and authenticity by verifying Intel's signature over the report.
\end{itemize}


% Requirement: If a user marks a device as a \textit{Remember this device}, then the device should not be compromised at that time. It can be compromised anytime after that. This assumption can be removed in specific scenarios and is discussed in SEC[EXPLAIN SGXIO AND OTHER ideas]

% \ks{I'm not fully understanding this yet so we should discuss. Is this an assumption we make for writing the paper to simplify the discussion. I know remember this device, but what does trusted device mean?}
% \tarun{Moved this from the threat model to System design section. This is a requirement that we need for our system to work. Because in case a user marks a device as "Remember this device", and the client is compromised at that time, the attacker can mark their device to be remembered instead of the user's device. Do we need to add the explanation here why we need this requirement? I think it would be hard to explain it here before explaining how we are implementing "Remember this device" feature. May be we can put this at the end of our analysis as limitation?}
% \ks{Yes, let's try this as a limitation.}




\subsubsection{The Relying Party}
% \paragraph{Registration Acknowledgement}
Currently, the \hsk assumes a completed registration as soon as it sends the response to the webAuthn client. We propose that the \rp returns an acknowledgment of successful registration to the \hsk after receiving a valid registration response. The acknowledgment contains the hash of the \hsk response.


Algorithm 3 in Appendix~\ref{sec_algorithm} shows the registration/authentication process at the \rp when a user initiates to register/authenticate a \hsk. The \rp first attempts to attest the client's \ver, if successful uses \textit{v-FIDO2} system, otherwise uses the current FIDO2 system. In the \textit{v-FIDO2} system, the \rp sends an authenticated request and initializes the clone detection algorithm by inserting the \textit{challenge} in the buffer. On receiving the response, the \rp verifies the appended authentication code. If successful, the \rp registers/authenticates the \hsk and updates the buffer for clone detection. In case of registration, the \rp also sends back an authenticated ack.    

% \ks{Does this mean my hsk is sometimes doing advanced clone detection when v-FIDO2, but may have to do plain FIDO2 when I access a machine without a V. Do they work together? I guess the RP/hsk are both storing hashes for v-FIDO2 and counters for FIDO2?}
% \tarun{In the current algorithm, it doesn't use hashed counter detection for FIDO2. We can write the algorithm in such a way but I think it might complicate thing. But I can give it a try.}


\subsubsection{The WebAuthn Client}
\paragraph{Built-in hardware authenticator}
The verifier (\ver) provides a \textit{remember this device} feature that is resistant to a MITM attack. Once a user authenticates using an \hsk on a device they can enable a built-in \hsk that operates from within \ver. The user can avoid having to insert an \hsk for future logins from this device based on the \textit{remember this device} period. 
% \ks{Is this built-in device registered as any other hsk? Is this something the user manually does when this is created?}
% \tarun{Yes! it's registered as a regular \hsk, but the \rp maintains 2 separate list for external authenticators and internal authenticators. User doesn't have to do it manually, if the user marks the device to be remembered, in the background an another request is sent to the RP to register the background authenticator. Then the user need to do a key tap on their external \hsk to authenticate new hsk registration.}

The built-in \hsk is registered automatically in the background using the same process as a regular \hsk. However, the user needs to approve the built-in \hsk by tapping on the external \hsk. The \rp maintains separate lists for the external and built-in authenticators.

\ver creates a private-public key pair used for signing the challenges received from the \rp for authentication. \ver seals the private key, and only \ver can unseal that private key and authenticate. At the time of authentication, \ver first checks whether it has a sealed registered key before prompting the user to authenticate using their \hsk. If the \textit{remember this device} feature has been enabled, \ver uses the sealed key to authenticate automatically in the background.

\paragraph{Error messages}
Currently, the \rp assumes responsibility for displaying messages when errors occur during the registration or authentication process. From our analysis, \rp error messages are inconsistent and can be difficult for users to understand.
We propose that the webAuthn client be responsible for displaying FIDO2 error messages based on standardized error codes and error messages that the \rp returns to the webAuthn client when an error occurs. 
This approach may be more usable by providing consistent error messages across all {\rp}s.

For example, when an \rp detects \hsk cloning, it can return a standard \emph{Device cloning detection} error code to the webAuthn client that results in standard error messages such as "Your security key may have been cloned. An attacker may have accessed your account. Remove the security key from this account and re-register it in order to lock out the attacker."

Algorithm 4 in Appendix~\ref{sec_algorithm} describes the process of \ver. In \textit{v-FIDO2}, the WebAuthn client acts as a relay for \hsk-to-\ver and \ver-to-\rp communications, where \ver runs on a TEE. On receiving a request, \ver verifies the HMAC using key $sk1$ and the origin specified in the request. If successful, it forwards the authenticated request (with a different key $sk2$) to \hsk and then acts as a relay between \rp and \hsk for authenticated communication between them.


\subsubsection{The Hardware Security Key}
\paragraph{Adding a security key display}
We propose a display screen on the \hsk to involve the user to help prevent some critical attacks (see Threat Analysis in Section~\ref{analysis}). 
During registration, the \hsk displays information and asks the user to confirm the registration process. We use webAuthn's Simple Transaction Authorization Extension (txAuthSimple), which allows us to display a string to the user for registration authorization. A Relying Party can specify a prompt string, intended for the \hsk's display.

On receiving a registration request, the \hsk displays four pieces of information.
(1) the \rp name, 
(2) the Username, 
(3) First authenticator indicator-- to show whether an \hsk is already bound to this account, and (4) Secure enclave indicator-- to prevent a downgrade attack from v-FIDO2 to FIDO2 when the client has a TEE.
The user taps the \hsk to confirm the details before the \hsk generates the response and sends it to the \rp. 

After successful registration, \rp responds with an ack that contains a hash of the \hsk response. \hsk verifies the hash, and if it matches, \hsk displays successful registration; otherwise, it shows a warning. The registration acknowledgment prevents cuckoo attacks because if an attacker uses their TEE and \hsk, the user's \hsk will not receive an acknowledgment that it can verify. If the \rp shows successful registration on the client's display and there is no successful registration acknowledgment on \hsk display, the user should consider it an attack.

On receiving an authentication request, the \hsk displays two pieces of information.
(1) the \rp name, 
(2) Secure enclave indicator.
The user taps the \hsk to confirm the details before the \hsk generates the response and sends it to the \rp. 

\paragraph{Additional authenticator registration}
To prevent a double-binding attack during a registration or authenticated session, we propose that an \rp requires the user to authenticate the use of an existing \hsk before adding another \hsk to an account. It prevents an attacker from registering a fake \hsk in the background without the user's knowledge.



% \paragraph{Algorithm 5} describes the registration/authentication process on \hsk. The \hsk attest the \ver and use that key (sk2) to verify the authenticated messages from \ver. Before creating the registration response, the \hsk displays the important details on the \hsk display. After verifying the details, the users tap the /hsk and allow \hsk to create a registration response and forward it to \ver. After getting an ack from the \ver the \hsk displays a "successful registration" message on the display. In case of an authentication request, display remains empty and the user just need to tap to verify presence. The \hsk also updates the clone detection hash value. 

Algorithm 5 in Appendix~\ref{sec_algorithm} specifies the registration/authentication process on the \hsk. The \hsk attests \ver to create key $sk2$ to authenticate messages from \ver. Upon receipt of the registration request, the \hsk displays the details. After verifying the details, the user taps the \hsk to instruct it to create a registration response and forward it to \ver. After receiving an ack from \ver, the \hsk displays a "Successful Registration" message. Upon receipt of an authentication request, the display remains empty, and the user taps to verify presence. The \hsk also updates the clone detection hash value. 

% \paragraph{Implementation}
% We created a prototype implementation of v-FIDO2 using an Intel SGX Enclave module. The details of the prototype implementation are in Appendix~\ref{prototype}.

\subsubsection{Discussion}

This section discusses v-FIDO2 design issues requiring further exploration and limitations.

\textit{Remote attestation scalability}  The authenticated messages in the v-FIDO2 are achieved using remote attestation. Remote attestation depends on a third-party attestation service. However, a popular web service, with high authentication traffic, can setup a local attestation infrastructure for Intel SGX to avoid making an external RPC for every request.


\textit{ Usability affect and support for non-SGX users}
% In our design, the TEE is optional to provide additional security, but 
 If a client doesn't support a TEE, the FIDO2 protocol works as usual. 
 When a user initiates FIDO2 authentication, the \rp sends an attestation request to the client. If a TEE is not supported, the client returns a response to fallback to the legacy protocol. The user verifies the "Secure enclave Indicator" on \hsk display to ensure that a malicious webAuthn client doesn't fall back to the legacy protocol when the client supports a TEE.
% \input{Discussion}

\textbf{\textit{Limitations}} The v-FIDO2 design has several limitations.
First, the v-FIDO2 design has a high deployment cost by requiring changes in all three entities--- browser, \rp, and \hsk. Second, v-FIDO2 relies on TEE, which some client machines may not have. Third, {\em remember this device} in v-FIDO2 prevents the passive cookie-stealing attack by using the built-in authenticator. However, there is no way to authenticate the built-in \hsk in v-FIDO2. Therefore, if a user marks a compromised device to be remembered, the adversary can mark their device to be remembered instead of the victim's device. Due to this risk, a high-value user should avoid using this feature. Fourth, TEEs like SGX and TrustZone are vulnerable to side-channel attacks.\cite{cerdeira2020sok} \cite{van2018foreshadow} \cite{cloosters2020teerex}. Fifth, our proposed system lacks a usability study. Our research opens up avenues for future usability research in cloning warning messages, registration notifications, and \hsk displays interactions.  


==> Threat_analysis.tex <==
\subsection{v-FIDO2 Security Analysis}
\label{analysis}

The v-FIDO2 design has \rp and \hsk authenticate \ver using remote attestation. 
\ver authenticates RP using the existing web PKI infrastructure (i.e., web server certificate). 
This authentication results in \rp and \hsk each sharing a key with \ver that they use to authenticate messages to and from \ver (e.g., HMAC). The user receives an authenticated confirmation message on their \hsk display to confirm successful registration at the intended \rp (i.e., domain name) under the correct username.

% \st{To confirm that the user's \hsk was registered at the correct \rp, the user receives a confirmation message on their \hsk display. The user can confirm the registration completed at the intended \rp (i.e., domain name) under the correct username.
% The shared keys with \ver guarantee the integrity of this confirmation.}

% \st{In the remainder of this section, we discuss each attack presented in the threat model and describe how the system design mitigates the attack.}


This section discusses each attack and describes how the v-FIDO2 design mitigates the attack. Table~\ref{attacks-defense} shows the attacks, attack type, and v-FIDO2 mitigations. Appendix~\ref{app:security_analysis}  (1) presents proof of how v-FIDO2 provides integrity and mitigates protocol flaws, \textit{Theorem 2: Assume adversary \A controls all the entities on webAuthn request/response flow except \ver, \hsk, and \rp. If the victim verifies the information shown on the \hsk display during registration/authentication, \A cannot modify a webAuthn request/response without being detected}, and (2) discusses how v-FIDO reduces the likelihood of social engineering attacks due to an HCI flaw.

% \begin{theorem}Integrity of FIDO2 messages: 
% Assume adversary \A controls all the entities on webAuthn request/response flow except \ver, \hsk, and \rp. If the victim verifies the information shown on the \hsk display during registration/authentication, \A cannot modify a webAuthn request/response without being detected. 
% \end{theorem}

% \begin{theorem}Integrity of FIDO2 messages: 
% Assume adversary \A controls all the entities on webAuthn request/response flow except \ver, \hsk, and \rp. If the victim verifies the information shown on the \hsk display during registration/authentication, \A cannot modify a webAuthn request/response without being detected. 
% \end{theorem}

% \begin{proof}
% In v-FIDO2, both \rp and \hsk perform remote attestation of \ver to (1) establish a shared key with \ver for message authentication, (2) ensure \ver is an authentic TEE, and (3) verify the integrity of the code running in \ver.
% After attestation, \rp and \hsk share $sk_1$ and $sk_2$, respectively, with \ver. They use these keys to generate an HMAC on each request/response sent/received from \ver to ensure the integrity of messages between \rp and \hsk.

% For authentication, \A has to allow communication to the victim's \hsk because the registration keys are in the victim's \hsk. Victim verification of the secure enclave indicator and the \rp name on the \hsk display ensures they are using v-FIDO2 and authenticating to the intended \rp.

% By design, the victim verifies the following four pieces of information on the \hsk display during registration: (1) \rp name, (2) username, (3) first authenticator indicator, and (4) secure enclave indicator. 
% Verifying the \rp name ensures the victim's \hsk is registered on the intended \rp, and verifying the username ensures the correct account at the \rp. Verifying the first authenticator indicator confirms whether an \hsk is already bound to this account. Verifying the secure enclave indicator ensures registration used v-FIDO2. Finally, the victim verifies the registration acknowledgment to ensure that the registration of the victim's \hsk succeeded. A parallel registration request to register \A's \hsk is infeasible because the first authenticator indicator ensures that \A has not already registered their \hsk in the background. \A cannot register its authenticator second because that first requires authentication from the victim's \hsk. 
% % To ensure that victim's \hsk interact with victim's intended \rp, victim verifies they get an acknowledgement during registration and verifies all four fields shown on the \hsk during registration
% \end{proof}

% \paragraph{HCI flaw}
% In section ~\ref{sec:flaw_user_misunderstanding}, we described three types of user misunderstandings that lead because of HCI flaw. First, Attacks 1b, 2b, and 3b result in an attacker registering their \hsk on the user's account because of vague notification. v-FIDO2 prevents attacks 1a, 2a, and 3a, removing the need for registration notification to detect the attacks. Second, Attack 5b describes bypassing the clone detection algorithm due to a vague error message. Our proposed clone detection algorithm and clear error messages about the attack resolve it. None of the 10 {\rp}'s we analyzed mention a cloning attack in their cloning detection error messages (see Table~\ref{rp-analysis}). We believe this is a limitation, and future work is needed to design effective error messages.

% Third, attacks 6 and 7 are feasible because there is no way for a user to verify for which \rp the \hsk is signing the authentication request when they tap the \hsk. Confirming the \rp on the \hsk display ensures that the \hsk is signing the request for the intended \rp. In the future, we plan to do an in-depth user study to design an effective clone detection error message and study the usability of verification of info on an \hsk display.



%\input{attacks_and_defenses_table}

% \subsection{Man-in-the-middle Attacks}

%\paragraph{Mis-binding attack during registration}
\paragraph{Attack 1}

The attacker modifies the \hsk response to register a fake \hsk. Under the new design, the authenticated message channel between the \hsk and \ver and between \ver and \rp provide message integrity and allow \ver or \rp to detect any modification to the response. If the adversary modifies the webAuthn response transmitted from \hsk to \ver, \ver detects it using the HMAC.


% If an adversary A3 (with WebAuthn client access), A2 or A3 modifies the registration response from \ver to \rp, there would be HMAC mismatch on the response \rp receives.


% There are two variants of the attack where the adversary may attempt to circumvent the authenticated message defense.
The adversary may attempt to circumvent the authenticated message defense by redirecting the registration request to an adversary-controlled \ver. In this case, an attacker could register the fake \hsk with the \rp. However, the victim does not receive a registration acknowledgment on their \hsk's display, allowing the victim to detect the attack immediately. Also, the user's \hsk display shows the victim username and \rp domain during registration, preventing the attacker from imitating the registration acknowledgment by binding to an incorrect \rp or username.
    
% The adversary can try a variant of this attack by allowing the registration request to the user's \hsk but dropping the registration response. Then, the webAuthn client initiates the second registration request and redirects it to adversary controlled \ver. This imitates the registration behavior at the user's \hsk and the attacker successfully registers their \hsk. But this attack would also be detected as the user would not get the registration acknowledgment from the \rp, so the victim's \hsk does not display a registration confirmation.

%  \textit{(2) The attacker impersonates the victim and binds the original \hsk with another account to imitate key registration behavior at the user's \hsk}: The adversary registers a fake \hsk with the user's account and, in parallel, registers the user's \hsk with a fake \rp or a fake account under another username at the intended \rp. This parallel fake request imitates the registration behavior at the user's \hsk. The victim receives notification that an \hsk was registered and sees an \hsk registered on the account. However, authentication will fail the next time the user authenticates to the account using the \hsk. The user's \hsk display helps prevent the attack by having a user verify that the \hsk is binding with the correct \rp and username. 
% \end{itemize}
\input{defenses_table}

%\paragraph{Double-binding  attack  during  registration}
\paragraph{Attack 2, 3}
% In this double-binding attack, both the user's \hsk and a fake \hsk are bound to the user's account during registration. If a fake \hsk is bound first, the user detects it by the {\em is First Authenticator} value being false on their \hsk display.
% The adversary cannot bind the fake \hsk second because our design requires the user to first authenticate using a registered \hsk, which is owned by the user. The authenticated channel between the \rp and \hsk via \ver ensures the integrity of the messages i.e the value of {\em is First Authenticator} would be accurate. 

% This attack can also be detected in the current FIDO2 protocol if the RP sends a notification on every \hsk registration that highlights the make \&\ model of the \hsk and the total number of registered {\hsk}s.

v-FIDO2 detects an attacker's attempt to register a fake \hsk and the victim's \hsk during registration. If the fake \hsk is registered first, the user detects it by the {\em is First Authenticator} value being false on their \hsk display.
If the attacker attempts to register the fake key second during registration (Attack 2) or it attempts to register their \hsk in the background (Attack 3), the system requires the attacker to authenticate using the registered user's \hsk first.
The integrity guarantee of the v-FIDO2 messages prevents an attacker from interfering with user notifications. 

These attacks can also be detected in the current FIDO2 protocol if the RP sends a notification on every \hsk registration highlighting the \hsk make \&\ model and the total number of registered {\hsk}s.

%\paragraph{Double-binding attack during authenticated session}
% \paragraph{Attack 3}
% An attacker attempts to register their \hsk in the background. Requiring the user to re-authenticate using a registered \hsk while adding a new \hsk prevents the attack.

%\paragraph{Signing algorithm downgrade attack}
\paragraph{Attack 4}
The attacker modifies the request message sent from the \rp to the \hsk. 
The integrity of the FIDO2 messages enables the \hsk or \ver to detect the attack.

% \tarun{Clone detection claim: Assume a user U authentications to RP using an HSK. If an attacker A clones U's HSK, and successfully authenticates to RP at least one time, U and RP detect the clone attack as soon as U tries to authenticate to RP. }

%\paragraph{Device cloning}
\paragraph{Attack 5}
v-FIDO2 relies on a Hashed Challenge List for device clone detection. The RP maintains an ordered list of hashes of challenges sent to the \hsk. The \hsk returns the challenge saved from the most recent authentication, which an \rp will accept only once. After cloning, whichever device authenticates first will include the stored hash, causing a clone detection error whenever the second device eventually authenticates. The \rp will always be made aware of the error, and the user will receive the clone detection error message if their \hsk authenticates second. 

% \st{The v-FIDO2 design uses a Hashed Challenge Set for device clone detection. The RP and the user's \hsk maintain a set of the synchronized hash of challenge. When the attacker uses the cloned \hsk they update the hash on the RP end. The user detects it on the next login attempt due to a mismatch in the clone detection hashes. The \textit{Hashed Challenge Set} ensures the detection of stealthy device cloning because the attacker cannot update the hash value with a future challenge hash, like incrementing the counter.}

% \st{The v-FIDO2 design uses a Hashed Challenge Set for device clone detection. The RP maintains a set of past hashed challenges that it expects to contain the next hash a legitimate \hsk will submit. When the attacker authenticates with a cloned \hsk, the hash set is re-initialized with the hash sent to the clone \hsk. When the legitimate user attempts to login to the \rp, a mismatch is detected. The \textit{Hashed Challenge Set} ensures the detection of stealthy device cloning because the attacker cannot update the stored hash value on the real \hsk with a future valid challenge hash, similar to simply incrementing the counter in the current FIDO2 design.}


%\paragraph{Synchronized login attack}
\paragraph{Attack 6, 7}
The user verifies \rp's domain name on the \hsk display. If the \hsk receives an authentication request from an \rp where the user is not actively logging in, the user should decline to tap the key indicating user presence. Without the tap, the \hsk does not generate an authentication response. Also, our design relocates the origin verification code to \ver so \A cannot circumvent it.

% \subsection{Phishing Attack}

%\paragraph{Coordinated MITM attack}
% \paragraph{Attack 4, 5}
% In the coordinated attack, the phishing site lies about the origin of the \rp to the \hsk, with assistance from a compromised webAuthn client. 
% Our design relocates the origin verification code to \ver, so it cannot be circumvented. 

% \st{The attack will be prevented by \ver.}

%\paragraph{Authentication method downgrade attack}
%\paragraph{Attack 7}

%Standard error codes and error messages can help train users on proper security behavior and may trigger cautious behavior when something unexpected occurs.  
%For instance, an authentic error code that requests a user downgrade the authentication method can include a cautious warning such as ``Verify that you are visiting the correct website. You are downgrading your secure login method."
%However, the system cannot prevent a phishing website from displaying messages on a web page that coerce a victim into providing a weaker form of authentication that can be more easily exploited than FIDO2.


%\paragraph{Cookie-stealing attack}
\paragraph{Attack 8}
When a user designates a device "to be remembered," \ver registers itself as a built-in \hsk on the account. 
The \rp stores the public key, and the associated private key is stored on \ver and sealed using the SGX sealing feature. Only \ver can access the sealed key on the device.

Using a built-in \hsk in secure hardware is more secure than passwords, cookies, or shared keys because it preserves the strengths of the authenticator approach (phishing attack resistance, MITM attack prevention, etc.). Unlike cookies, there is no data for an eavesdropper to steal and replay to impersonate the user. Also, the TEE prevents malware from accessing the private key. However, it is less secure than the \hsk as it does not require user presence, and a malicious client can automatically authenticate as the user through the user's device. This design reduces the attack surface. To impersonate the user, an attacker must compromise the webAuthn client and attempt impersonation from the user's device. 

% \tarun{Built-in \hsk is a stronger defense against man-in-the-middle network attackers compared to cookies. Like cookies, built-in HSKs should also have an expiration value, possibly limiting the damage in case of a compromised client.}

% The design replaces cookie authentication with FIDO2 authentication using a built-in \hsk. The user accesses their physical \hsk only during registration and whenever the \textit{remember this device} period expires. In subsequent logins, authentication occurs automatically in the background, similar to cookie authentication. However, there is no message data that an eavesdropper can steal and replay as in the cookie-stealing attack. This design reduces the attack surface. To impersonate the user, an attacker must compromise the webAuthn client and attempt impersonation from the user's device. 


% There are two use cases
%     Organization (Fixed set of relying parties)        
%         Hardcode RP's public keys in the secure enclave
%             User's authenticator needs to have ISV's public key (most likely RP's in this case)
%             RP needs to have ISV's public key (most likely RP's in this case)

%     General Users 
%         The user's authenticator needs to have ISV's public key.

\subsection{Discussion on v-FIDO2} \tarun{New section}
The necessary changes required for v-FIDO2 implementation involve hardware security keys (HSKs), browsers, and FIDO2 libraries. The practicality of v-FIDO2 as a security enhancement for FIDO2 is possible because all of these three entities are actively involved in FIDO2 progression. Therefore, it is feasible to adopt v-FIDO2 before widespread adoption of FIDO2.

Furthermore, v-FIDO2 can be an opt-in protocol, allowing high-value targets and new adopters with compatible machines (TEE) to purchase hardware tokens with displays for additional security, while others can continue to use the legacy protocol. This incremental user adoption approach allows for a smoother transition to v-FIDO2.

Although there are limitations to TEE security, researchers are working to improve its security. The v-FIDO2 protocol does not depend on a specific secure enclave and can utilize future developments in TEE technology. Until then, v-FIDO2 raises the bar on attackers, as breaking secure enclaves is more complex than browser extension or malware attacks.

Finally, even if v-FIDO2 is not widely adopted, it provides a baseline that researchers can use to compare future proposals. The research impact of v-FIDO2 lies in its potential to inspire further advancements in hardware security key technology and browser security, making it a valuable addition to the field of authentication security.







\subsection{Implementation summary}
We created a prototype implementation of v-FIDO2 using an Intel SGX Enclave module. When a user initiates a registration request, the client initializes the enclave and launches the verifier (\ver).
The \rp and \hsk both attest to {\ver}'s validity using the remote attestation feature of Intel SGX. 
The result of attestation is that \ver shares a secret key with \rp and \hsk, respectively. The keys are used to authenticate messages sent between them. More details of the implementation are presented in Appendix ~\ref{prototype}.

% \subsubsection{WebAuthn client and Verifier (\ver)}
% The webAuthn client acts as a relay for \hsk-to-\ver and \ver-to-\rp communications. 
% We implemented the webAuthn client in two modules: (1) \textit{browser extension}, responsible for overriding the current FIDO2 browser webAuthn client and acting as a relay between \rp and the webAuthn client's native C++ app, and (2) native C++ app using Yubico's libfido2 library that initializes \ver and acts as a relay for webAuthn client's browser extension-to-\ver and \ver-to-\hsk communication. We implemented the Intel SGX module ~\ver within the native application. More details of the implementation are presented in Appendix ~\ref{prototype}.
 
    % Native app's APIs that are available to the Chrome extension/RP are (1) remote attestation of the ~\ver: The remote attestation process provides the ~\ver and the Relying Party with the shared secret key (Sk), (2) registers an ~\hsk: If the remote attestation is successful, the input to this API is encrypted by Sk. The ~\ver decrypts the request and re-encrypts it with the secret key shared with the ~\hsk, (3) authentication: same process as registration API.
        
    % There is only one native app's API available to the authenticator. The app allows the authenticator to attest to the Verifier's secure enclave. The app also sends the IAS report to the authenticator that helps the authenticator complete the attestation process. The Verifier communicates with the authenticator over an encrypted channel by using the secret key they shared during attestation.  



% \begin{figure*}[b]
% % [htbp]\centerline{\includegraphics{SGX_FIDO2_implementation.png}}
% \includegraphics[width=0.97\textwidth,height=0.62\textwidth]{SGX_FIDO2_implementation.png}
% \caption{Communication flow in v-FIDO2 implementation}
% \label{system_overview}
% \end{figure*}

% \subsubsection{Hardware Security Key (\hsk)}

% In our design, the \hsk uses a modified version of the Intel SGX remote attestation process to verify that it communicates to a valid enclave. Typically a portion of this process requires the service provider, the system requesting proof of an enclave, to connect to the IAS and receive an attestation report. Since the \hsk cannot connect directly to the IAS, the enclave itself retrieves the attestation report and forwards it to the \hsk. The \hsk then verifies the report using the hard-coded IAS public key on the device. This process provides evidence to the \hsk that it authenticated to a genuine SGX enclave and that the enclave is running a valid copy of \ver. After the remote attestation process completes, each message sent between the \hsk and \ver running on the SGX is authenticated using a shared key generated during remote attestation.

% \subsubsection{Relying Party (\rp)}

% The \rp also uses remote attestation to verify it is talking to a valid SGX that is running a valid copy of \ver, resulting in a shared key between \rp and \ver. 
% \rp authenticates all messages sent from \ver using that shared key. \rp also sends an acknowledgment after registration or authentication completes successfully.
% In our prototype, we build upon Yubico's \textit{java-webauthn-server} repository to implement our server. On the server, we implemented a separate module $RP checker$. Its primary job is to verify the \ver secure enclave through remote attestation and share a secret key $Sk$. It also communicates with the \textit{IAS} to retrieve the attestation report. After successful attestation, $RP checker$ shares the key $Sk$ with the $RP$. The WebAuthn server uses $Sk$ to generate an HMAC of the request and includes it in the registration or authentication request.

\subsubsection{Performance analysis}
% \tarun{In progress}

In v-FIDO, the computation and network overhead are mainly due to remote attestation. This section presents the performance overhead  (see Table~\ref{tab:performance}) to establish shared keys and include an HMAC on each webAuthn request/response.

\paragraph{Remote attestation}
In v-FIDO2, \rp and \hsk each perform remote attestation to establish shared keys with \ver. 
An attestation may occur only once if the key is cached for future authentication.
 In our design, \rp connects to IAS to verify the {\ver}'s attestation signature from Intel and obtain the attestation certificate. \rp passes this attestation certificate to \hsk through \rp. To calculate the computation and network overhead due to remote attestation, we computed the average of 1,000 remote attestation trials.

\textit{Delay:}
 Attestation of \ver by \rp and \hsk takes 1.094 sec and 0.243 sec resp. Attestation verification takes, on average, 0.84 secs (out of 1.094 secs). \hsk receives the attestation certificate from \rp through the client, and it just needs to perform attestation and verify with the attestation certificate. 
Overall, this results in a 1.337 sec delay while performing remote attestation during webAuthn registration or authentication.
We believe this delay will not significantly affect usability because the webAuthn registration and authentication wait for the user to tap the \hsk.

\textit{Network traffic:}
\rp adds 31.1 KB of total network traffic for remote attestation where 21 KB of network traffic is from IAS verification, and \rp sends 5.6 KB IAS report to \hsk ). Because \hsk does not need to perform IAS verification, it only adds 10.27 KB consisting of 4.57 KB for remote attestation and 5.6 KB for receiving an IAS report. The network traffic for \hsk is the additional data it sends/receives to/from the client. \hsk does not connect to the Internet.
The client involves in remote attestation with \rp and \hsk; therefore, the total additional network traffic because of remote attestation is 20.27 KB (4.5 KB + 4.57 KB + 2*5.6KB).


\paragraph{Memory}
\rp, \hsk, and \ver must cache the symmetric keys if they do not want to perform remote attestation repeatedly. \rp and \hsk store a 32-byte key per client. \rp and \hsk also store Intel SGX Attestation root CA's public key (1.9 KB) to authenticate the IAS report. Finally, the client seals the symmetric keys to secure them. The memory cost to seal two 32-byte keys is 614 bytes.

\paragraph{WebAuthn registration/authentication network traffic}
v-FIDO2 only adds HMAC to requests and responses. The total additional network traffic for \rp and \hsk are 64 bytes each because they both receive and send an additional 32-byte HMAC on request and responses. The client relays both the requests and responses; therefore, it sends/receives an additional 128 bytes during webAuthn registration and authentication.
% \paragraph{}

% Total network data for remote attestation from \rp: 4,538 bytes (tcpdump -> capinfos from wireshark-common package. )

% 25.5 = 21 kB (IAS verification) + 4.538kB (remote attestation)

% 32 bytes for HMAC


% Average total time taken: 1.094 seconds (used 'time' command to calculate time for executable)

\input{performance_table}

% ip.addr == 40.87.90.88

% https://geek-university.com/measure-time-of-program-execution/)
% Memory used on \rp: 32 byte (key size)





==> duplicate_references.tex <==
@inproceedings{chakraborty2019simfido,
  title={simFIDO: FIDO2 User Authentication with simTPM},
  author={Chakraborty, Dhiman and Bugiel, Sven},
  booktitle={Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security},
  pages={2569--2571},
  year={2019}
}

@inproceedings{zhang2015trusttokenf,
  title={Trusttokenf: A generic security framework for mobile two-factor authentication using trustzone},
  author={Zhang, Yingjun and Zhao, Shijun and Qin, Yu and Yang, Bo and Feng, Dengguo},
  booktitle={2015 IEEE Trustcom/BigDataSE/ISPA},
  volume={1},
  pages={41--48},
  year={2015},
  organization={IEEE}
}

@article{costan2016intel,
  title={Intel SGX Explained.},
  author={Costan, Victor and Devadas, Srinivas},
  journal={IACR Cryptol. ePrint Arch.},
  volume={2016},
  number={86},
  pages={1--118},
  year={2016}
}

@article{rijswijk2013using,
  title={Using trusted execution environments in two-factor authentication: comparing approaches},
  author={Rijswijk-Deij, Roland van and Poll, Erik},
  journal={Open Identity Summit 2013},
  year={2013},
  publisher={Gesellschaft f{\"u}r Informatik eV}
}

@article{bhargav2014trusted,
  title={TRUSTED EXECUTION ENVIRONMENT FOR PRIVACY PRESERVING BIOMETRIC AUTHENTICATION.},
  author={Bhargav-Spantzel, Abhilasha},
  journal={Intel Technology Journal},
  volume={18},
  number={4},
  year={2014}
}

@incollection{paladi2017safeguarding,
  title={Safeguarding vnf credentials with intel sgx},
  author={Paladi, Nicolae and Karlsson, Linus},
  booktitle={Proceedings of the SIGCOMM Posters and Demos},
  pages={144--146},
  year={2017}
}

@inproceedings{will2020using,
  title={Using a Shared SGX Enclave in the UNIX PAM Authentication Service},
  author={Will, Newton C and Maziero, Carlos A},
  booktitle={Proceedings of the 14th Annual International Systems Conference, Montreal, QC, Canad{\'a}. IEEE},
  year={2020}
}

@inproceedings{conde2018using,
  title={Using Intel SGX to Protect Authentication Credentials in an Untrusted Operating System},
  author={Cond{\'e}, Rafael CR and Maziero, Carlos A and Will, Newton C},
  booktitle={2018 IEEE Symposium on Computers and Communications (ISCC)},
  pages={00158--00163},
  year={2018},
  organization={IEEE}
}

@inproceedings{shah2015multi,
  title={Multi-factor Authentication as a Service},
  author={Shah, Yogendra and Choyi, Vinod and Subramanian, Lakshmi},
  booktitle={2015 3rd IEEE International Conference on Mobile Cloud Computing, Services, and Engineering},
  pages={144--150},
  year={2015},
  organization={IEEE}
}

@inproceedings{o2019min,
  title={MIN () imum Failure:$\{$EMFI$\}$ Attacks against $\{$USB$\}$ Stacks},
  author={O'Flynn, Colin},
  booktitle={13th $\{$USENIX$\}$ Workshop on Offensive Technologies ($\{$WOOT$\}$ 19)},
  year={2019}
}

==> performance_table.tex <==
\begin{table}
	\centering
	\caption{Performance analysis}
	\label{tab:performance}
	\begin{tabular}{l|p{0.7cm}|p{1cm}|c|c|p{1.2cm}}
		              & \multicolumn{2}{c|}{Remote attestation}        &   \multicolumn{2}{c|}{Memory}    &                         Reg/Auth overhead                  \\
		\textit{Entity}  & Total time & Network Traffic  & per \rp & one time & Network Traffic                        \\
		\midrule

		\rp  & $1.09$ s                            &  $31.1$ KB     & $32$ B     & $1.9$ KB       & $64$ B     \\
		
		\hsk  & $0.24$ s              & $4.57$ KB                & $32$ B     & $1.9$ KB  &     $64$ B                 \\

%     	KTCA  & < 2 epochs ($1$ epoch + $2\cdot(diam(G) $+$1)\cdot\delta$)                            & $104 B$                       & $7.136 KB$                                & $1.056 KB$     & $1.056 KB$      \\
    	


% 		AKM      & <$m$ epochs ($\approx10^\ddagger$ epochs)                            & $0$                           & $~32 KB$                                 & $~320 KB$  & $~320 KB$            \\

		
% 		KTACA                        &  <1 epoch +$\Delta$                      & $104 B$                     & $33.96 KB$                                 & $1.056 KB$ & $1.056 KB$            \\
		
		
		
% 		\midrule
% 		&  Waiting time & & & & \\
% 		\midrule
		
% 		Prevention mode                   & $+0$(new key), $2\cdot\delta$ (key update) & $+4.8 KB$                     & $+0$                                 & $+0$    & $40 KB$\textsuperscript{\textdagger}         \\
		



	\end{tabular}
	
	
	
	\vspace{3mm}
    % $\ddagger$~ = the delay is after the beginning of the next epoch in which the contact starts communication~~~~~~~

    
    
    
    % \textdagger~= Detection time is for detection mode, and waiting time is for prevention mode. The waiting time in prevention mode is presented as <new connections, existing connections>.\\
% 	\textdagger~= Using TOR service as the out-of-band channel, the actual data exchanged is 64 bytes~~~~~~~
% 	$\ddagger$~ = detects with $0.999$ probability\\
    % $+$~ = in addition to the corresponding value of a defense that includes prevention mode
    


% 	\detects~detects the attack, \partialp~sometimes prevents the attack \\
\end{table}

==> prototype.tex <==

\subsection{v-FIDO2 Prototype Implementation}
\label{prototype}
When a user initiates a registration request, the client initializes the enclave and launches the verifier (\ver).
The \rp and \hsk both attest to {\ver}'s validity using the remote attestation feature of Intel SGX. 
The result of attestation is that \ver shares a secret key with \rp and \hsk respectively. The keys are used to authenticate messages sent between them.


\subsubsection{Prototype Implementation Details}
We created a prototype implementation of v-FIDO2 using an Intel SGX Enclave module. When a user initiates a registration request, the client initializes the enclave and launches the verifier (\ver).
The \rp and \hsk both attest to {\ver}'s validity using the remote attestation feature of Intel SGX. 
The result of attestation is that \ver shares a secret key with \rp and \hsk respectively. The keys are used to authenticate messages sent between them.

%\subsubsection{Background: Intel SGX}
Intel SGX is a set of CPU instructions that can be used by applications to create an isolated region of memory called an enclave. The enclave is inaccessible to everyone outside the enclave, including processes with admin privileges and the operating system. 
The application that creates an enclave is divided into a trusted and untrusted section. The untrusted section is responsible for creating an enclave and communicating with the rest of the system. 
%The untrusted section uses ECALLs to invoke a pre-defined function, passing input parameters and pointers to shared memory in the enclave. The enclave uses OCALLs to invoke functions outside the enclave by copying input parameters outside the enclave.
    
\paragraph{Remote attestation}
Remote attestation guarantees the integrity of the trusted code in the enclave. When an ISV (Independent Software Vendor) develops the application, they generate a cryptographic hash (known as MRENCLAVE) of the running enclave, including both the code and data of the trusted section. 
The ISV shares the hash with service providers that need to attest to the enclave of that application. A service provider challenges an enclave to generate a MRENCLAVE and compares it with the MRENCLAVE provided by the ISV.
To verify that the MRENCLAVE is created by a legitimate enclave instance, it must be signed with the enclave's private key. Relying parties send the signature to the IAS (Intel Attestation Service) for verification.

\subsubsection{WebAuthn client and Verifier (\ver)}

We implemented \ver as an Intel SGX module based on code provided at \url{https://github.com/intel/sgx-ra-sample}. 
The webAuthn client acts as a relay for \hsk-to-\ver and \ver-to-\rp communications. 
We implemented the webAuthn client in two modules: (1) \textit{browser extension}, responsible for overriding the current FIDO2 browser webAuthn client and acting as a relay between \rp and the webAuthn client's native C++ app. Please note this extension only relays the messages with MAC, and an attacker cannot execute any attack if they compromise this extension.(2) native C++ app that initializes \ver and acts as a relay for webAuthn client's browser extension-to-\ver and \ver-to-\hsk communication.


 We implemented webAuthn client as a native C/C++ application using Yubico's libfido2 library. We implemented the Intel SGX module ~\ver within the native application based on code provided at https://github.com/intel/sgx-ra-sample. The ~\ver uses v2.7 of Intel's SGX driver, SDK, and Platform Software(PSW). This native application initializes \ver and acts as a relay for \rp-to-\ver and \ver-to-\hsk communication. . It communicates to the ~\hsk using the CTAP protocol implemented in the libfido2 library. To allow the app's communication to an RP through a web browser, we implemented a Chrome extension. The Chrome extension overrides the inbuilt $navigator.credentials.create()$ and $navigator.credentials.get()$ functions, and calls the native app implementation. 
 
    Native app's APIs that are available to the Chrome extension/RP are (1) remote attestation of the ~\ver: The remote attestation process provides the ~\ver and the Relying Party with the shared secret key (Sk), (2) registers an ~\hsk: If the remote attestation is successful, the input to this API is encrypted by Sk. The ~\ver decrypts the request and re-encrypts it with the secret key shared with the ~\hsk, (3) authentication: same process as registration API.
        
    There is only one native app's API available to the authenticator. The app allows the authenticator to attest to the Verifier's secure enclave. The app also sends the IAS report to the authenticator that helps the authenticator complete the attestation process. The Verifier communicates with the authenticator over an encrypted channel by using the secret key they shared during attestation.  



\subsubsection{Hardware Security Key (\hsk)}

In our design, the \hsk uses a modified version of the Intel SGX remote attestation process to verify that it is communicating to a valid enclave. Typically a portion of this process requires the service provider, the system requesting proof of an enclave, to connect to the IAS and receive an attestation report. Since the \hsk cannot connect directly to the IAS, the enclave itself retrieves the attestation report and forwards it to the \hsk. The \hsk then verifies the report using the IAS public key that is hard-coded on the device. This process provides evidence to the \hsk that it is authenticated to a genuine SGX enclave and that the enclave is running a valid copy of \ver. After the remote attestation process is completed, each message that is sent between the \hsk and \ver running on the SGX is authenticated using a shared key that is generated during the remote attestation process.

\subsubsection{Relying Party (\rp)}
The \rp also uses remote attestation to verify it is talking to a valid SGX that is running a valid copy of \ver, resulting in a shared key between \rp and \ver. 
\rp authenticates all messages sent from \ver using that shared key. \rp also sends an acknowledgement after registration or authentication completes successfully.
In our prototype, we build upon Yubico's \textit{java-webauthn-server} repository to implement our server. On the server, we implemented a separate module $RP checker$. Its primary job is to verify the \ver secure enclave through remote attestation and share a secret key $Sk$. It also communicates with the \textit{IAS} to retrieve the attestation report. After successful attestation, $RP checker$ shares the key $Sk$ with the $RP$. The WebAuthn server uses $Sk$ to generate an HMAC of the request and include it in the registration or authentication request.

